Properties of the `friend of a friend' model for network generation

The way in which a social network is generated, in terms of how individuals attach to each other, determines the properties of the resulting network. Here we study an intuitively appealing `friend of a friend' model, where a network is formed by each newly added individual attaching first to a randomly chosen target and then to $n_q\geq 1$ randomly chosen friends of the target, each with probability $0<q\leq1$. We revisit the master equation of the expected degree distribution for this model, providing an exact solution for the case when $n_q$ allows for attachment to all of the chosen target's friends (a case previously studied by \cite{lambiotte2016}), and demonstrating why such a solution is hard to obtain when $n_q$ is fixed (a case previously studied by \cite{Levens2022}.) In the case where attachment to all friends is allowed, we also show that when $q<q^*\approx0.5671$, the expected degree distribution of the model is stationary as the network size tends to infinity. We go on to look at the clustering behaviour and the triangle count, focusing on the cases where $n_q$ is fixed.

==> removed.tex <==

\subsubsection{Worst case scenario for the clustering coefficient}
Here, we consider a scenario where the same node is selected and a link is established with the new node at each time of the network growth. At each step, we calculate the maximum number of triangles in $G$ containing the target node $v$ (max $E_{v}$). 
\begin{enumerate}
    %\item When a new person joins the network and establishes friendships with %$n_q$ neighbours of a degree $k$ target $v$, the number of new triangles formed %by this new person with the existing network is given by what distribution? %Maybe this \[\frac{n_q(n_q-1)}{2}\]
    \item Case 1: $n_q =1$. When a new node is connected to an already existing node $v$, both the degree of $v$ and $E_v$ are incremented by $1$. Thus, \[E_v = k-1\]
\item Case 2: $n_q =2$. For a sequence of time $t_0, t_1, t_2, t_3, t_4, ...$, a corresponding sequence of max $E_{v}$ represented as a function of $k$ is given by
\[k+1, k+2, k+3, k+4, k+5,...\]
The nth term of this sequence can be written as a function of $k$ and $n_q$ as
\begin{equation} \label{E_v1}
  \text{max} E_{v(n_q\le2,k)} = n_q(k-1)-(n_q-1) = n_q(k-2)+1 
\end{equation}
Eq. \ref{E_v1} works for cases 1 and 2. 
\item Case 3: Higher order $n_q = 3,4,5,...$. By numerical simulation, we trace how the max $E_{d_i}$ changes with the increase in $n_q$ as shown in Table \ref{sequenceEk}. 

\begin{table}[h!]
\caption{Table for the difference between max $E_{v}$ for the network generated by second order $n_q = 2$ and other higher-orders $n_q = 3,4,5,...$}
\label{sequenceEk}
\centering
 %\begin{tabular}{||c c c||} 
 \begin{tabular}{ |p{2.5cm}|p{6.2cm}|p{5cm}| }
 \hline
 Higher order $n_q$ & $d_i=n_q-2=$ Higher order-Second order & max $E_{d_i} =E_{v_{n_q = 2}}-E_{v_{n_q = 3,4,5,...}}$ \\ [0.5ex] 
 \hline
 3 & 1 & 1 \\ 
 4 & 2 & 3 \\
 5 & 3 & 6 \\
 6 & 4 & 10 \\
 7 & 5 & 15 \\  
  . & . & . \\ 
   . & . & . \\ 
    . & . & . \\ [1ex]
 \hline
 \end{tabular}
\end{table}
As shown in Table \ref{sequenceEk}, $d_i$ gives the variable for the terms of the sequence max $E_{d_i}$ in the last column. 
The nth term $E_d$ for max $E_{d_i}$ is given by 
\begin{equation}\label{edi}
E_d = \frac{1}{2}d_i^2+\frac{1}{2}d_i= \frac{1}{2}(n_q-2)^2+\frac{1}{2}(n_q-2).
\end{equation}
The quantity $E_d$ gives the excess number of triangles in $G$ containing the target node $v$ for $\text{Max}  E_{v(n_q\le2,k)}$ at each time step. Thus, subtracting Eq.\ref{edi} from Eq.\ref{E_v1} gives the general formula for max $E_v$:
\begin{equation}\label{generalEv}
    \text{max} E_{v(n_q,k)} = \text{max} E_{v(n_q\le2,k)}-E_d = n_q(k-1/2)-\frac{1}{2}n_q^2
\end{equation}

\item Now, considering the probability q of linking with each neighbour, what is the probability of forming $E_k$ when the new person joins the network?
\item Local clustering coefficient $C_v = \frac{2E_v}{k_v(k_v-1)}$
\item Clustering coefficient of a node with degree $k$ is given by,\[
		C_k= \frac{\left[ P_k(t)qn_q + qn_q \frac{k \cdot P_k(t)}{2(1+qn_q)} \right]E_v}{\left[ P_k(t) + qn_q \frac{k \cdot P_k(t)}{2(1+qn_q)} \right](k(k-1)/2)} 
\]
\end{enumerate}

\note{Tiffany: Is this result interesting enough?? Also, it is for $n_q\geq 2$. I tried to do it more generally but didn't get further.   }

